Zodiacal Exoplanets in Time (ZEIT) II. A "Super-Earth" Orbiting a Young K Dwarf in the Pleiades Neighborhood

We describe a "super-Earth"-size ($2.30\pm0.15R_{\oplus}$) planet transiting an early K-type dwarf star in the Campaign 4 field observed by the K2 mission. The host star, EPIC 210363145, was identified as a member of the approximately 120-Myr-old Pleiades cluster based on its kinematics and photometric distance. It is rotationally variable and exhibits near-ultraviolet emission consistent with a Pleiades age, but its rotational period is ~20 d and its spectrum contains no H$\alpha$ emission nor the Li I absorption expected of Pleiades K dwarfs. Instead, the star is probably an interloper that is unaffiliated with the cluster, but younger (< 1 Gyr) than the typical field dwarf. We ruled out a false positive transit signal produced by confusion with a background eclipsing binary by adaptive optics imaging and a statistical calculation. Doppler radial velocity measurements limit the companion mass to <2 times that of Jupiter. Screening of the lightcurves of 1014 potential Pleiades candidate stars uncovered no additional planets. An injection-and-recovery experiment using the K2 Pleiades lightcurves with simulated planets, assuming a planet population like that in the Kepler prime field, predicts only 0.8-1.8 detections (vs. ~20 in an equivalent Kepler sample). The absence of Pleiades planet detections can be attributed to the much shorter monitoring time of K2 (80 days vs. 4 years), increased measurement noise due to spacecraft motion, and the intrinsic noisiness of the stars.

==> setup.tex <==
%% For anyone who downloaded my source file from arxiv:
%% I stole most of this setup.tex from a paper by Peter .K.G. Williams, but I made a bunch of edits to satisfy my own needs. You might check his paper out (http://arxiv.org/abs/1409.4411) for the original source file or contact him if you have any questions, since I don't really understand how some of these things work. 
%One cool thing it does is you can define an object, just that when someone clicks on the pdf it will link to simbad. I could never quite get this to work, probably because you have to get the text exactly right and my motivation for getting it to work was not super high. 


% basic packages
\usepackage{amsmath,amssymb}
\usepackage[breaklinks,colorlinks,urlcolor=blue,citecolor=blue,linkcolor=blue]{hyperref}
\usepackage{epsfig}    
\usepackage{graphicx}    
\usepackage{lineno}
\usepackage{natbib}
\usepackage{bigints}
\usepackage[outdir=./]{epstopdf}



% font stuff
\usepackage[T1]{fontenc}
\pwifjournal\else
  \usepackage{microtype}
\fi


% emulateapj has overly conservative figure widths, I think because some
% people's figures don't have good margins. Override.
\pwifjournal\else
  \makeatletter
  \renewcommand\plotone[1]{%
    \centering \leavevmode \setlength{\plot@width}{0.95\linewidth}
    \includegraphics[width={\eps@scaling\plot@width}]{#1}%
  }%
  \makeatother
\fi


% My amazing object-referencing system!
%
% \MakeObj[shortname]{ident}{url-escaped name}{formal name}
%    defines an object
% \MakeTrunc{ident}{truncname}
%    defines a truncated name for a blended object (e.g. LP 349-25 *AB*)
%
% \obj{ident}:  link using standard/short name
% \objf{ident}: link using formal/full name
% \objt{ident}: link using the truncated name
%
% Links are \object{} commands if in journal mode, links to Simbad otherwise.
%
% Under the hood:
%
% \pkgwobj@c@<ident> turns its argument into an appropriate link for the object
% \pkgwobj@f<ident>  expands into the formal/full name of the object
% \pkgwobj@s<ident>  expands into the standard/short name of the object

\makeatletter

\newcommand\@simpfx{http://simbad.u-strasbg.fr/simbad/sim-id?Ident=}

\newcommand\MakeObj[4][\@empty]{% [shortname]{ident}{url-escaped}{formalname}
  \pwifjournal%
    \expandafter\newcommand\csname pkgwobj@c@#2\endcsname[1]{\protect\object[#4]{##1}}%
  \else%
    \expandafter\newcommand\csname pkgwobj@c@#2\endcsname[1]{\href{\@simpfx #3}{##1}}%
  \fi%
  \expandafter\newcommand\csname pkgwobj@f#2\endcsname{#4}%
  \ifx\@empty#1%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#4}%
  \else%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#1}%
  \fi}%

\newcommand\MakeTrunc[2]{% {ident}{truncname}
  \expandafter\newcommand\csname pkgwobj@t#1\endcsname{#2}}%

\newcommand{\obj}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@s#1\endcsname}%
  \fi}
\newcommand{\objf}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@f#1\endcsname}%
  \fi}
\newcommand{\objt}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@t#1\endcsname}%
  \fi}

\makeatother


% Evil magic to patch natbib to only highlight the year paper refs, not the
% authors too; as seen in ApJ. From
% http://tex.stackexchange.com/questions/23227/.

\pwifjournal\else
  \usepackage{etoolbox}
  \makeatletter
  \patchcmd{\NAT@citex}
    {\@citea\NAT@hyper@{%
       \NAT@nmfmt{\NAT@nm}%
       \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
       \NAT@date}}
    {\@citea\NAT@nmfmt{\NAT@nm}%
     \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}
  \patchcmd{\NAT@citex}
    {\@citea\NAT@hyper@{%
       \NAT@nmfmt{\NAT@nm}%
       \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
         {\@citeb\@extra@b@citeb}%
       \NAT@date}}
    {\@citea\NAT@nmfmt{\NAT@nm}%
     \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
    {}{}
  \makeatother
\fi




% utility

